Intersection Types and (Positive) Almost-Sure Termination

Randomized higher-order computation can be seen as being captured by a lambda calculus endowed with a single algebraic operation, namely a construct for binary probabilistic choice. What matters about such computations is the probability of obtaining any given result, rather than the possibility or the necessity of obtaining it, like in (non)deterministic computation. Termination, arguably the simplest kind of reachability problem, can be spelled out in at least two ways, depending on whether it talks about the probability of convergence or about the expected evaluation time, the second one providing a stronger guarantee. In this paper, we show that intersection types are capable of precisely characterizing both notions of termination inside a single system of types: the probability of convergence of any lambda-term can be underapproximated by its type, while the underlying derivation's weight gives a lower bound to the term's expected number of steps to normal form. Noticeably, both approximations are tight -- not only soundness but also completeness holds. The crucial ingredient is non-idempotency, without which it would be impossible to reason on the expected number of reduction steps which are necessary to completely evaluate any term. Besides, the kind of approximation we obtain is proved to be optimal recursion theoretically: no recursively enumerable formal system can do better than that.

==> 04-CharacterizationCF.tex <==
% !TEX root = main_PAST.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Characterizing Probabilistic Termination}\label{sec:characterization}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section presents the main result of this paper, namely the
characterisation of both forms of probabilistic termination by
typing. This will be done by relating type derivations for a program
$M$ with the probability of termination and the expected runtime of
$M$. To achieve the latter, we need to focus on \emph{tight}
derivations, since not all type derivations of $M$ underapproximate
the expected runtime of $M$.

We show that in the tight case, $\ETime M$ (respectively, $\ProbTerm{M}$)
bounds from above the weight $w$ (resepectively, the norm
$\norm{\at}$) of any type derivation $\Pi\dem\oder{w}{M:\at}$. This is
the \emph{soundness property}, and is in Section~\ref{sec:sound}. We also
prove the converse, \ie the \emph{completeness property}, in Section~\ref{sec:complete}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tight Typings}
%%%%%%%%%%%%%%%%%%%%%%%%%%
The need for tight typings can be grasped easily by considering
the following example
\begin{example}\label{ex:tight}
  The term $I$ is in normal form, and therefore $\ETime I=0$. It
  can be given the type $\zero$ (by way of the $\TZero$ typing rule),
  or the type $\mdist{1[]}$ (by way of $!$ and $\TVal$).
  In both cases, the underlying weight is $0$.
  However, $I$ also admits derivations whose weight is
  strictly positive, such as
  \[
  \infer[\lam]{\oder 1 \lam x.x: []\arrow []}{\infer[\TVar]{x:[] \oder 0 x:[]  }{}}
  \]
  More generally, without any restrictions on the shape of types,
  one can easily assign grossly overapproximated weights to
  terms, e.g., the term $\lambda x.(\Delta\Delta)$, which is a value
  but which can receive arbitrarily large weights when given the
  type $[]\arrow\zero$, (immediate consequence of the example in  Section \ref{sec:too_little} above).
\end{example}
The purpose of arrow types is to give types to terms which are
\emph{not} supposed to be reduced alone, but only when applied
to an argument. If, instead, a term is not supposed to be used
as a function, its type must be the empty multiset. This is the
key idea for understanding the following definition:

\begin{Def}[Tight Types and Derivations]
  A type $\at$ is said to be \emph{tight} if it is a multidistribution
  on the empty intersection type $[]$. Accordingly, a derivation
  $\Pi\dem ~ \oder w M: \at $ is said to be \emph{tight} if $\at$ is tight.
\end{Def}
A tight type has therefore shape $\at=\mdist{q_k[]}_{\kK}$, where $K$ is
possibly nonempty. In particular the null type $\zero$ is a tight type. Observe that if
$\at$ is tight, then $\norm {\at}=\sum_k q_k$ (which, again, is null when $K$
is empty). The following can be proved by quickly inspecting the typing
rules:
\begin{lemma}[Tight Typings for Values] \label{lem:normalV}
  If $V$ is a closed value, then there
  are precisely two tight derivations for $V$, both of weight $0$:
\[
\infer[\TVal]{\oder 0 V:\mdist{1[]}}{\infer[!]{\oder 0 V:[]}{}} \quad\quad  \infer[\TZero]{\oder 0 V:\zero}{}
\]
\end{lemma}
Looking back at Example \ref{ex:tight}, one immediately realizes that
tightness allows us to get rid of overapproximations, at least for values. Does
this lift  to all terms? The next two subsections will give a positive
answer to this question. The following  property, which is immediate from the definitions,
will be useful in the rest of this section.
\begin{property}\label{fact:approximants}
  For any closed term $M$ and any  $k\in \Nat$, it holds that
$\eval k M \leq \eval {k+1} M$ and $\etime k M \leq \etime {k+1} M$. Moreover, if $M\red \mdist {q_iM_i}_{\iI}$ then
\[
\eval {k+1} M = \sum_{\iI} q_i(\eval {k} {M_i}),\qquad
\etime {k+1} M = 1+ \sum_{\iI} q_i(\etime{k} {M_i}).
\]
\end{property}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Soundness}\label{sec:sound}
%%%%%%%%%%%%%%%%%%%%%%%
In this section, we prove the correctness of our type system. Namely,
we prove that if $\oder w M: \at$ is (tightly) derivable, then $M$ has
probability of termination at least $\norm \at$, and expected runtime
at least $w$.
  
The proof of correctness is based on the following, namely a form of
weighted subject reduction, that for good reasons has a probabilistic
flavor here.  The size of a type derivation $\Pi$ (denoted $\size
\Pi$) is the standard one, and is defined as the number of rules in
$\Pi$, (excluding the !-rule and the $\TVal$-rule, which cannot be
iterated.)

\begin{lemma}[Weighted Subject Reduction]\label{lem:SubRed}\label{lem:WSR}
   Suppose that $\Pi\dem \oder{w} P:\bt$, with $w >0$, and that $P \red
  \mdist{q_iP_i}_{\iI}$. Then for every $\iI$ there exists a
  derivation $\Pi_i$ such that $\Pi_{i}\dem\oder {w_i} P_i: \bt_{i}$,
  and $\size{\Pi} > \size{\Pi_i}$. Moreover,
%  \begin{enumerate}
%  \item
    $\bt= \dsum_{i\in I} q_i \bt_{i }$ and 
%  \item
    $w=1+ \sum_{i\in I} q_i w_i$.		
%  \end{enumerate}
\end{lemma}
\SLV{The proof is in the extended version.}{The proof is in the Appendix.}
Notice how the type stays \emph{the same}, at least on the average,
while the weight strictly \emph{decreases}. This in turn implies that whenever
a term is (tightly) typable, its weight is a lower bound to its expected
time to termination, while the norm of its type is a lower bound to the
probability of termination. This is proved by way of approximations, as
follows:
\begin{theorem}[Finitary Soundness ]\label{th:correct}
  Let $M$ be a \emph{closed} term.  For each tight typing $\oder w M:
  \bt$, there exists $k\in \Nat$ such that
%  \begin{enumerate}
  %\item
  $ \norm \bt \leq \eval k M$  and %(\ie 	after $k$ steps, $M$   is in normal form with probability \emph{at least}  $\norm \bt$);
%\item
  $w \leq \etime k M $.
%    (\ie 	the expected runtime of  $M$   is \emph{ at least}  $w$).
%  \end{enumerate}	
\end{theorem}


%\begin{theorem}[Tight Correctness - finitary]\label{th:correct} Let $M$ be  a \emph{closed} term and 
%	  $\Pi\dem ~ \oder w M: \bt$ be a \emph{tight} derivation. Then there exists    
%	 $k\in \Nat$ such that 
%	\begin{enumerate}
%		\item  $ \norm \bt \leq \nnorm {\m}$ with   $\mdist{M}\Red^k \m$\\  (\ie 	after $k$ steps, $M$   is in normal form with probability \emph{ at least}  $\norm \bt$);
%		\item $w \leq \etime k M $\\
%		 (\ie 	the expected runtime of  $M$   is \emph{ at least}  $w$).
%	\end{enumerate}	
%\end{theorem}

\begin{proof}
  By induction on the size $\size{\Pi}$ of the type derivation $\Pi$
  such that $\Pi\dem\oder w M$, distinguishing some cases. Recall that for closed terms,  the normal forms are exactly  the values. 
  \begin{varitemize}
  \item
    If $M$ is a value, the claim holds by Lemma \ref{lem:normalV}, where we observe that  $w=0$. 
    Notice that  $\eval 0 M =\nnorm {\mdist{M}}=1$ and   
    $\etime 0 M=0$.
  \item
   Otherwise, if $M$ is not a value,  we further distinguish some cases:
    \begin{varitemize}
    \item If $w=0$, then by inspecting the rules, we see that the only
      derivable tight judgment is $\oder 0 M:\zero$ which trivially
      satisfies the claim, with $k=0$.
    \item If $w>0$, then since $M$ is not normal, it has a reduction
      step $M \red \mdist{q_iM_i}_{\iI}$.  By Weighted Subject
      Reduction (Lemma \ref{lem:WSR}), we derive that for each $\iI$
      there exists a derivation $\Pi_i \dem \oder{w_i} M_i:\bt_i$,
      with $\size {\Pi_i} <\size {\Pi}$. Since $\bt$ is tight,
      necessarily each $\bt_i$ also is tight, again by
      Lemma~\ref{lem:WSR} (observe also that, if $\bt=\zero$, then
      $\bt_i=\zero$).  By \ih, for each $M_i (\iI)$ there exists
      $k_i\in \Nat$ which satisfies the conditions on $\norm{\bt_i}$
      and $w_i$.  Let $h=max \{k_i\}_{\iI}$.  Since ${h}\geq k_i$, for
      each $\iI$ we have $\norm {\bt_i} \leq \eval {h} {M_i}$ and $w_i
      \leq \etime{h} {M_i}$.  Moreover, Weighted Subject Reduction
      implies also that $ \norm \bt =\sum_i q_i \norm {\bt_i}$ and $w=
      1 + \sum_i q_i w_i$.  The claim follows easily by
      Property~\ref{fact:approximants}, with $k=h+1$. Indeed $\eval
      {h+1} M = \big(\sum_{\iI} q_i \eval {h} {M_i}\big) \geq \big(
      \sum_{\iI} q_i \norm{\bt_i}\big)= \norm{\bt}$ and $\etime {h+1}
      M = \big(1+ \sum_{\iI} q_i \etime {h} {M_i}\big) \geq \big(1+
      \sum_{\iI} q_i w_i \big)= w$.
    \end{varitemize}
  \end{varitemize}
  Since there are no other cases, we are done.
\end{proof}
Observe that Theorem~\ref{th:correct} holds for every tight type $\bt$, including the null type. Thus it has 
the following immediate consequence:
\begin{cor}[Finitary Soundness of Null Typing]\label{cor:zero_correct}
  Let $M$ be a \emph{closed} term such that $\oder w M:
  \zero$. Then there exists $k\in \Nat$ such that $w \leq \etime k M$.
\end{cor}
%This implies that if we are only interested in correctness for the
%expected runtime --and not the probability of termination-- we can
%just focus on the type $\zero$.

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Completeness}\label{sec:complete}
%%%%%%%%%%%%%%%%%%%%%%%%%
The last section showed that type derivations provide lower bounds on
the probability of convergence, and on the expected time to
termination. It is now time to prove that \emph{tight} derivations
approximate \emph{with arbitrary precision} the aforementioned
quantities.  The proof of completeness is based on the following
probabilistic adaptation of Weighted Subject Expansion, whose proof is
 in \SLV{the extended version.}{the Appendix.}
\begin{lemma}[Weighted Subject Expansion]\label{lem:SubEx}
  Let $P$ be a closed term.  Assume that $P\red \mdist{q_i P_i}_{\iI}$ and
  that for each $\iI$, $\Pi_i \dem \oder {w_i} P_i:\at_i $. Then, there exists a
  single derivation $\Pi\dem \oder {w} P:\at $ such that $\at=\dsum_i
  (q_i\at_i)$ and $w\geq 1+\sum q_i w_i$.
\end{lemma}
We can now thus prove the dual to Theorem~\ref{th:correct} above:
\begin{theorem}[Finitary Completeness]\label{th:complete}
  Let $M$ be a closed term.  For each $k\in \Nat$ there exists a
  \emph{tight} derivation $\Pi\dem ~ \oder w M:\at$, such that $\norm
  \at = \eval k M$ and $w \geq \etime k M $.
\end{theorem}
\begin{proof}
	By induction on $ k$, distinguishing some cases.
        \begin{varitemize}
	\item  If $M$ is a value, then for each $k$,  $\eval k M=1$ and $\etime k M =0$.   The  derivation 
	$\oder 0 M:\mdist{1[]}$ ( Lemma~\ref{lem:normalV}) satisfies the claim. 
	\item Otherwise, if $M$ is not a value: 
	\begin{varitemize}
		\item If $k=0$, we have  $\eval 0 M=0 = \etime 0 M$; the 
		 $\TZero$-rule satisfies the claim.

		\item
		If $k>0$, assume $M\red \mdist{p_i M_i}_{\iI}$.  
%		For
%		concreteness (but w.l.o.g.), let us discuss the instance
%		$I=\{1,2\}$, $p_i=\two$.  From $M\red \mdist{\two M_1, \two M_2}
%		\full^{k-1} \m$ we have that $\m=\m_1\uplus\m_2$, with
%		$\mdist{M_i}\full^{k-1}\m_i$, and $\nnorm \m= \two \nnorm {\m_1} +
%		\two \nnorm {\m_2}$. 
 By \ih, for each $i\in I$, there
		exists a tight derivation $\Pi_i\dem ~ \oder {w_i} {M_i}: \at_i$, such
		that $\norm {\at_i}=\eval {k-1}{M_i}$ and $w_i \geq  \etime {k-1}{M_i}
		$. By Weighted Subject Expansion, there exists a tight derivation
		$\Phi\dem \oder {w} M: \at $ such that $\norm {\at}=  \sum_{\iI} p_i \norm {\at_i} $, and $w\geq  \sum_{\iI}p_iw_i$. We conclude  by Property~\ref{fact:approximants}, because 
	 	  $\eval k M =  \sum_{\iI}	p_i	\eval {k-1} {M_i}  = \sum_{\iI}	p_i	\norm{\at_i}=\norm \at$
	 and 
	  $\etime k M = 1+ \sum_{\iI}	p_i	\etime {k-1} {M_i}  \leq 1+ \sum_{\iI}	p_i	w_i = w$.
	\end{varitemize}
\end{varitemize}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Various Flavours of a Correspondence}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\W}[1]{\mathbf{W}(#1)}
\newcommand{\N}[1]{\mathbf{N}(#1)}
This section is devoted to characterisation results
relating typing and termination. The latter can be given in three
different ways, and we devote a subsection to each of them.

\subsubsection{A Uniform Characterization}
%\paragraph{A Uniform Characterization}
A characterization of both $\ProbTerm M$ and $\ETime M$
by \emph{the same class} of derivations, namely tight
derivations, can be given as follows:
\begin{thm}[Tight Typing and Termination]\label{th:term_tight}\label{thm:characterization}
  Let $ M$ be a closed term.  Then
  \begin{align*}
  \ProbTerm M &= \sup  \{ \norm {\at}\st \exists\Pi.\Pi\dem  \vdash M:\at \mbox{ is a tight derivation} \}\\
  \ETime M  &=  \sup \{w  \st\exists\Pi,\at.\Pi\dem  \oder w M: \at \mbox{ is  tight derivation} \}
  \end{align*}
\end{thm}
\begin{proof} 
  Let us first of all define $\N{M}$ and $\W{M}$ as follows:
  \begin{align*}
    \N{M}&\deff \sup \{ \norm {\at}\st \Pi\dem  \vdash M:\at \mbox{ is a tight derivation } \}\\
    \W{M}&\deff \sup \{w  \st \Pi\dem  \oder w M: \at \mbox{ is  tight derivation } \}
  \end{align*}
  We now proceed by proving the following two statements:
  \begin{varitemize}
  \item
    On the one hand, we prove that 
    $ \N M = \ProbTerm M $, recalling that $\ProbTerm M :=\sup\{\eval n M\st n\in\Nat \} $. 
    \begin{varitemize}
    \item
      Let $ \Phi\dem \oder {} M: \at$ be a tight derivation. By
      Correctness (Theorem \ref{th:correct}), $\norm \at \leq
      \ProbTerm M$. Hence $\N M\leq \ProbTerm M$.
    \item
      By Finitary Completeness (Theorem \ref{th:complete}), for each $k\in
      \Nat$ there exists a tight derivation $\Pi \dem \oder {} M: \at
      $ such that $\eval k M \leq  \norm \at$.  Hence $\N M= \ProbTerm M$.
      %	Hence  $\ProbTerm M \leq \N  M$.
    \end{varitemize}
  \item 	
    On the other hand, we prove that 
    $\W M = \ETime M $, recalling that $\ETime M  := \sup\{ \etime n M\st n\in\Nat \}$ .     
    \begin{varitemize}
    \item
      Let $w $ be the weight of a tight derivation $ \Phi\dem \oder w
      M: \at$. By Correctness (Theorem \ref{th:correct}), $ w\leq
      \ETime M $. Hence $\W M\leq \ETime M$.
    \item
      Again by Finitary Completeness (Theorem \ref{th:complete}), for each $k\in
      \Nat$ there exists a tight derivation $\Pi \dem \oder w M: \at $
      such that $\etime k M \leq w$.  Hence $\W M= \ETime M$.
      %Hence	$\ETime M \leq \W M$.
    \end{varitemize}
  \end{varitemize}
  
\end{proof}

By definition, $M$ is \AST iff $\ProbTerm{M}=1$, while $M$ is \PAST iff $ \ETime M$ is finite; therefore  

\begin{cor}[Tight Typing, \AST, and \PAST] \label{cor:char_tight}
  Let $ M$ be a closed term. Then:
    $M$ is \AST iff $ \sup \{ \norm {\at}\st\exists\Pi.\Pi\dem \vdash M:\at
    \mbox{ is a tight derivation } \} =1 $. Moreover, 
    $M$ is \PAST iff $ \sup \{w \st\exists\Pi,\at.\Pi\dem \oder w M: \at \mbox{ is
    tight derivation } \} < \infty $.
\end{cor}

\newcommand{\ww}{\mathbf{w}} \newcommand{\oh}{\mathbf{v}}
\begin{example}

<<<<<<< .mine
\newpage


	\begin{example}
		\newcommand{\ww}{\mathbf{w}}
				\newcommand{\oh}{\mathbf{v}}


		In Section~\ref{sec:examples_CbV} we have   discussed  tight derivations for our running example $\mex\mex$. Each derivation $\Sigma_i$ ($i\in \Nat$) of $\mex$ has constant  weight $2$. Collecting and scaling the $j$  derivations $\Sigma_j, ..., \Sigma_1$ we  obtain $\Phi_j$ which has weight 
		$\ww_j =2(1+\two + ... + \frac{1}{2^{j-1}})= 2(\sum_{n<j} \frac{1}{2^n}) <4$.
	
		It is interesting to  sketch  also the type derivations for the terms $\cex\cex$ and $\expl{\cex\cex}$ of Example \ref{ex:succ}.
		
\begin{itemize}

\item 		We  can build a tight  type derivation  $\Sigma_i^\cex$ for  $\cex= \Big(\lam x.  ( \plett z {xx} {SUCC\, z})  \oplus \nzero \Big)$ by 
		following the blueprint of the derivations $\Sigma_i$ for $ \mex$.
		\gray{For example, 
		
		\[
		\Sigma_3^{\cex}\dem
		\infer{\ovdash{2+v_i} \lam x.  ( \plett z {xx} {SUCC\, z})     \oplus I: [\two \for\At_2, \frac{1}{4}\for \At_1]\arrow \dist{ \frac{1}{8}[], \frac{1}{4}[], \two []  }  }{
			\infer{  x:[\two \for\At_2, \frac{1}{4}\for \At_1] \ovdash{1+v_i} ( \plett z {xx} {SUCC\, z}) \oplus I:  
				\dist{ \frac{1}{8}[], \frac{1}{4}[], \two [] } }{
				\infer{x:[ \At_2, \two \for\At_1] \ovdash {1+c(\four+\two)} ( \plett z {xx} {SUCC\, z}) :    \dist{\frac{1}{4}[], \frac{1}{2}[]}  }{	
			z:[]\oder{c} \SUCC\, z : \mdist{[]}&		   z:[]\oder{c} \SUCC\, z : \mdist{[]} &\quad& {x:[ \At_2, \two \for\At_1] \ovdash  0 xx:    \dist{\frac{1}{4}[], \frac{1}{2}[]}  }
				}
				&
				\infer{\ovdash  0 I: \dist{[]}}{}
			}
		}
		\]
	%
		 The weight is now $2+v_i$, where 
		the  overhead $v_i$ is given by the left premisses of the $\letr$ rule and  depends on $SUCC$;   we have    $v_i = 1+ c(\two + ...+ \frac{1}{2^{i-1}}) $ %$(\sum_{n<i}{\frac{1}{2^{n}}})$
		 ($c\geq 1$ a constant).
		By collecting and scaling the  $j$  derivations $\Sigma_j^{\cex},\dots, \Sigma_1^{\cex}$ we can then obtain a type derivation $\Phi_j^{\cex\cex}$ for $\cex\cex$ (similarly to what we have done to obtain $\Phi_j$). The weight is now $\ww_j+  \oh_j$, where the overhead $\oh_j$ is obtained by summing  $v_j + \two v_{j-1}...., \frac{1}{2^{j-1}}v_1$ and so is bounded by $c(\sum_{n<j} \frac{1}{2^n}n) < 2c$.}

		
%			\pink{ An even more interesting term is $\eex$ of Example \ref{ex:succ}.  We can build a  tight derivation    $\Pi_j^{\eex}$ by 
%				 composing with a  derivation for $\cex\cex$. 
%				 One realizes that 
%			for each $j\in \Nat$, there is a tight type derivation whose weight exceeds  $\two \sum_{n<j} \frac{1}{2^n} \mathit{exp}(n) $. The set of such weights  is clearly unbounded.}

\item 	 An even more interesting term is $\expl{\cex\cex}$ of Example \ref{ex:succ}.  We can build a  tight derivation     for it  by 
	composing with a  derivation for $\cex\cex$. 
	
	First, it is clear  that  the term $\EXPL ~\overline n$ can be given a tight derivation of weight (proportional to) $\exp(n)$, in a standard way 
	\[\infer{ \der \EXPL~ \overline n : \mdist{[]}}{  \der \EXPL: \mA_n \arrow \mdist{[]}  & \der \overline n: \mA_n}\]
	
Now, observe that for each $j\in \Nat$,  we can build a type derivation for $\cex\cex$ which corresponds to producing the   natural numbers from $0$ to $j$. For example, for $j=2$ we have  $\oder{v}\cex\cex:  \mdist{   \two \mA_0, \four \mA_1,   \frac{1}{8}\mA_2}$.
We then can obtain  the following tight derivation
%
\[
\infer{\oder{w} \plett{z}{\cex\cex}{\EXPL~z}:  \two\mdist{[],   \two [], \frac{1}{2^2}[], \dots,  \frac{1}{2^{j}} []}
}
{ \Big(z:\mA_k  \oder{\mathit{exp}(n)}  \EXPL\, z:\mdist{[] } \Big)_{n\in \{0,\dots, j\}}
&
\oder{v}\cex\cex:  \two \mdist{\mA_0, \two \mA_1, \frac{1}{2^2}\mA_2, \dots,  \frac{1}{2^{j}} \mA_{j}  }
}
\]
where $w=\two \sum_{n:0}^j   \frac{1}{2^n}\mathit{exp}(n) +1+v$. 
	
	One realizes that 
	for each $j\in \Nat$,  $\expl{\cex\cex}$ has a tight type derivation whose weight exceeds  $\two \sum_{n:0}^j \frac{1}{2^n} \mathit{exp}(n) $, so  the set of tight weights  is clearly unbounded.

\end{itemize}
\end{example}

||||||| .r91
\CF{OPTIONAL -- }
\blue{
	\begin{example}
		\newcommand{\ww}{\mathbf{w}}
				\newcommand{\oh}{\mathbf{v}}
		In Section~\ref{sec:examples_CbV} we have   discussed  tight derivations for our running example $\mex\mex$. Each derivation $\Sigma_i$ ($i\in \Nat$) of $\mex$ has constant  weight $2$. Collecting and scaling the $j$  derivations $\Sigma_j, ..., \Sigma_1$ we  obtain $\Phi_j$ which has weight 
		$\ww_j =2(1+\two + ... + \frac{1}{2^{j-1}})= 2(\sum_{n<j} \frac{1}{2^n}) <4$.

		It is interesting to briefly sketch  also the type derivations for
		 the term $\cex\cex$ whose evaluation produces   countably many different  values  (Example~\ref{ex:evalCC}).
		%the terms $\cex\cex$ and $\eex$ of Example \ref{ex:succ}.
		


		We  can build a tight  type derivation  $\Sigma_i^\cex$ for  $\cex= \Big(\lam x.  ( \plett z {xx} {SUCC\, z})  \oplus \nzero \Big)$ by 
		following the blueprint of the derivations $\Sigma_i$ for $ \mex$. The weight is now $2+v_i$, where 
		the  overhead $v_i$ is given by the left premisses of the $\letr$ rule and  depends on $SUCC$;   we have    $v_i = 1+ c(\two + ...+ \frac{1}{2^{i-1}}) $ %$(\sum_{n<i}{\frac{1}{2^{n}}})$
		 ($c\geq 1$ a constant).
		By collecting and scaling the  $j$  derivations $\Sigma_j^{\cex},\dots, \Sigma_1^{\cex}$ we can then obtain a type derivation $\Phi_j^{\cex\cex}$ for $\cex\cex$ (similarly to what we have done to obtain $\Phi_j$). The weight is now $\ww_j+  \oh_j$, where the overhead $\oh_j$ is obtained by summing  $v_j + \two v_{j-1}...., \frac{1}{2^{j-1}}v_1$ and so is bounded by $c(\sum_{n<j} \frac{1}{2^n}n) < 2c$.

		
			\pink{ An even more interesting term is $\eex$ of Example \ref{ex:succ}.  We can build a  tight derivation    $\Pi_j^{\eex}$ by 
				 composing with a  derivations for $\cex\cex$. One realizes that 
			for each $j\in \Nat$, there is a tight type derivation whose weight exceeds  $\two \sum_{n<j} \frac{1}{2^n} \mathit{exp}(n) $. The set of such weights  is clearly unbounded.}

\end{example}}


%\pink{
%	\begin{example}
%		\newcommand{\ww}{W}
%	In Section~\ref{sec:examples_CbV} we have   discussed  tight derivations for our running example $\mex\mex$. Each derivation $\Phi_j$ ($j\in \Nat$) has weight $\ww_j =2\sum_{n<j} \frac{1}{2^n}$, which is bounded by $4$.
%It is interesting to briefly consider also type derivations for the terms $\cex\cex$ and $\eex$ of Example \ref{ex:succ}.
%
%\begin{itemize}
%	\item
%	 %The term $\cex\cex$ can be typed in a  similar way.   
%For the term $\cex\cex$, we already noticed that its evaluation (Example~\ref{ex:evalCC})   is similar to that of $\mex\mex$, but produces   countably many different  values.  We can build a  type derivation $\Phi_j^{\cex\cex}$ for $ \cex\cex$ 
%following the blueprint of the derivation $\Phi_j$ for $ \mex\mex$. Now instead of the $j$ leaves of shape  $\oder{0}I:\mdist{[]}$ we would have the $j$ tight type  derivations of
% $ \ssym^n ({\nzero})$ ($0\leq  n < j$), each 
%with respective weight $nK$. Taking into account  scaling, the weight of $\Phi_j^{\cex\cex}$ is then $\ww_j+
% \two K (\sum_{n<j} \frac{n}{2^n})  $. %Hence the set of weights is bounded by $4+K$.
% 
%\item  A tight type derivation   $\Phi_j^{\eex}$ for $\eex$ also can be build on the model of $\Phi$. Now the  leaves are replaced by  type  derivations of terms 
% $\expl{ \ssym^n ({\nzero})}$, each with weight  $v_n> \mathit{exp}(n)$; each such $v_n$ is then  scaled by $\two\frac{1}{2^n}$. Since for each $j\in \Nat$, there is a tight type derivation whose weight exceeds  $\sum_{n<j} \frac{1}{2^n} \mathit{exp}(n) $, the set of weights  is clearly unbounded.
%\end{itemize}
%	\end{example}}
=======
  In Section~\ref{sec:examples_CbV} we have discussed tight
  derivations for our running example $\mex\mex$. Each derivation
  $\Sigma_i$ ($i\in \Nat$) of $\mex$ has constant weight
  $2$. Collecting and scaling the $j$ derivations $\Sigma_j, ...,
  \Sigma_1$ we obtain $\Phi_j$ which has weight $\ww_j =2(1+\two +
  ... + \frac{1}{2^{j-1}})= 2(\sum_{n<j} \frac{1}{2^n}) <4$.  We can
  also sketch how type derivations can be built for the terms
  $\cex\cex$ and $\expl{\cex\cex}$ from Example \ref{ex:succ}:
  \begin{varitemize}
  \item
     We can build a tight type derivation $\Xi_i$ for $\cex=
     \Big(\lam x.  ( \plett z {xx} {SUCC\, z}) \oplus \nzero \Big)$ by
     following the blueprint of the derivations $\Sigma_i$ for $
     \mex$.
     %\gray{For example,
%
%       \[
%       \Sigma_3^{\cex}\dem
%       \infer{\ovdash{2+v_i} \lam x.  ( \plett z {xx} {SUCC\, z})     \oplus I: [\two \for\At_2, \frac{1}{4}\for \At_1]\arrow \dist{ \frac{1}{8}[], \frac{1}{4}[], \two []  }  }{
%         \infer{  x:[\two \for\At_2, \frac{1}{4}\for \At_1] \ovdash{1+v_i} ( \plett z {xx} {SUCC\, z}) \oplus I:  
%           \dist{ \frac{1}{8}[], \frac{1}{4}[], \two [] } }{
%           \infer{x:[ \At_2, \two \for\At_1] \ovdash {1+c(\four+\two)} ( \plett z {xx} {SUCC\, z}) :    \dist{\frac{1}{4}[], \frac{1}{2}[]}  }{ 
%             z:[]\oder{c} \SUCC\, z : \mdist{[]}&   z:[]\oder{c} \SUCC\, z : \mdist{[]} &\quad& {x:[ \At_2, \two \for\At_1] \ovdash  0 xx:    \dist{\frac{1}{4}[], \frac{1}{2}[]}  }
%           }
%           &
%           \infer{\ovdash  0 I: \dist{[]}}{}
%         }
%       }
%       \]
%       %
%       The weight is now $2+v_i$, where the overhead $v_i$ is given by
%       the left premisses of the $\letr$ rule and depends on $SUCC$;
%       we have $v_i = 1+ c(\two + ...+ \frac{1}{2^{i-1}}) $
     %       %$(\sum_{n<i}{\frac{1}{2^{n}}})$ ($c\geq 1$ a constant).
     By appropriately
       collecting and scaling the $j$ derivations
       $\Xi_j,\dots, \Xi_1$ we then obtain a
       type derivation $\Theta_j$ for $\cex\cex$ (similarly
       to what we have done to obtain $\Phi_j$). The weight is now
       bounded by $k(\sum_{n<j} \frac{1}{2^n}n) < 2k$.
   \item
     An even more interesting term is $\expl{\cex\cex}$.  We can build
     tight derivations for it by starting from the derivations
     $\Theta_j$. First, it is clear that the term $\EXPL ~\overline n$
     can be given a tight derivation of weight (proportional to)
     $2^n$, in a standard way.
%     \[
%     \infer{ \der \EXPL~ \overline n : \mdist{[]}}{  \der \EXPL: \mA_n \arrow \mdist{[]}  & \der \overline n: \mA_n}
%     \]
%     Now, observe that for each $j\in \Nat$, we can build a type
%     derivation for $\cex\cex$ which corresponds to producing the
%     natural numbers from $0$ to $j$. For example, for $j=2$ we have
%     $\oder{v}\cex\cex: \mdist{ \two \mA_0, \four \mA_1,
%       \frac{1}{8}\mA_2}$.  We then can obtain the following tight
%     derivation
%     \[
%     \infer{\oder{w} \plett{z}{\cex\cex}{\EXPL~z}:  \two\mdist{[],   \two [], \frac{1}{2^2}[], \dots,  \frac{1}{2^{j}} []}
%     }
%           { \Big(z:\mA_k  \oder{\mathit{exp}(n)}  \EXPL\, z:\mdist{[] } \Big)_{n\in \{0,\dots, j\}}
%             &
%             \oder{v}\cex\cex:  \two \mdist{\mA_0, \two \mA_1, \frac{1}{2^2}\mA_2, \dots,  \frac{1}{2^{j}} \mA_{j}  }
%           }
%     \]
%     where $w=\two \sum_{n:0}^j \frac{1}{2^n}\mathit{exp}(n)
%     +1+v$.  One realizes that for each $j\in \Nat$,
     %     $\expl{\cex\cex}$ has
     From then, for every $j$, a tight type derivation having weight
     at least $\two \sum_{n\leq j} \frac{2^n}{2^n}=\frac{j+1}{2}$ can be built,
     so the set of tight weights is clearly unbounded.
\end{varitemize}
\end{example}
>>>>>>> .r93

<<<<<<< .mine
\newpage

||||||| .r91

=======
>>>>>>> .r93

\subsubsection{Focusing on Expected Runtimes.}
Remember that $\PAST\subset\AST$.  The previous characterisation may
give the impression that analysing the runtime of a term somehow
requires studying its probability of termination.  In fact, our type
system allows us to establish \PAST \emph{independently} from \AST, by
looking only at the type $\zero$ rather than at \emph{all} tight
typings. The results we are going to prove tell us that if we are only interested in
the expected runtime, we can indeed \emph{limit the search space}
to the derivations of the null type $\zero$.  First of all,
a strengthening of Finitary Completeness can be given
 \begin{prop}[Finitary Completeness of Null Typing]\label{th:zero_complete}
   Let  $M$ be a closed term. 
%   \begin{enumerate}
%   \item For each derivation	$\Pi\dem ~ \oder w M: \zero$, there exists    
%     $k\in \Nat$ such that  $w \leq \etime k M$.
   %   \item
   Then, for each $k\in \Nat$ there exists a derivation $\Pi\dem ~
   \oder w M:\zero$, such that $w \geq \etime k M $.
%   \end{enumerate}
 \end{prop}
 \begin{proof} 
%   \begin{enumerate}
%   \item Immediate corollary of finitary correctness.
   % \item
   The proof is a simplification of Theorem \ref{th:complete}. We only
   need to observe  that the $\zero$ typing is preserved by subject
   expansion, and the weights strictly increases along it.
   \SLV{}{ As
     before,we prove the claim by induction on $ k$.
       \begin{varitemize}
       \item $k=0$. We have   $\etime 0 M=0$, and the $\zero$-rule satisfies the claim.
       \item $k>0$. Assume  $M\red \mdist{p_i M_i}_{\iI} \full^{k-1} \m$.  		
	 For concreteness (but w.l.o.g.), let us discuss the   instance $I=\{1,2\}$,
	 $p_i=\two$.
	 From   $M\red \mdist{\two M_1, \two M_2} \full^{k-1} \m$ we have that  $\m=\m_1\uplus\m_2$, with $\mdist{M_i}\full^{k-1}\m_i$. 	By \ih, for each  $i\in \{1,2\}$, 
	 there exists a  derivation   $\Pi_i\dem ~ \oder w_i M_i: \zero$, such that  $w_i = \etime {k-1}  {M_i} $. By
	 Weighted Subject Expansion,  there exists a   derivation  $\Phi\dem  \oder {w} M: \zero$ such that 
	 $w= \two w_1+ \two w_2+1$. This proves the claim,  because  $\etime k M = 1+ \two \etime {k-1} {M_1}  +  \two \etime {k-1} {M_2} = 1+  \two w_1+ \two w_2$.
       \end{varitemize}
     }%SLV
%   \end{enumerate}	
 \end{proof}
 Since Finitary Soundness holds at all types, we can easily reach
 the following:
\begin{thm}[Null Typing, Expected Runtimes, and \PAST]\label{thm:char_null}
  Let $ M$ be a closed term.  Then:
  $$
  \ETime M  =   \sup \{w  \st \Pi\dem  \oder w M: \zero \}\qquad
  M\in\PAST\Leftrightarrow\sup \{w  \st \Pi\dem  \oder w M: \zero \} < \infty
  $$
\end{thm}
%%%%%%%%%The proof is in the%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The Running Example, Revisited}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us go back to our running example $\mex\mex$, and show that its runtime
can be analysed by way of null types. We can indeed build type
derivations of the form $\Pi \dem \oder w \mex\mex:\zero$ in such a
way that $w$ is bounded by $\ETime {\mex\mex}=4$, and for each
approximant $\etime k {\mex\mex}$ there is a derivation which has at
least that weight.  The structure of these type derivations are
identical to the ones we gave in Section \ref{sec:examples_CbV}.  The
only difference is in how the underlying \emph{types} are defined.  Let us define
the families of types $\{\Bt_n\}_{n\in\Nat}$ and
$\{\mb_n\}_{n\in\Nat}$ as follows:
\begin{align*}
\mb_0= []\qquad\qquad
\mb_n =  \two\for \mb_{n-1} 	\uplus 	\two\for  [\Bt_n]\qquad\qquad
\Bt_n=   \mb_{n-1}\arrow  \zero
\end{align*}
For example:
\begin{align*}
\Bt_1&=[] \arrow \zero, & \Bt_2&=\mb_1\arrow  \zero, & \Bt_3&=\mb_2\arrow   \zero, \\
\mb_1 &=\mset{\two \for\Bt_1}&\mb_2 &= \mset{\frac{1}{4} \for\Bt_1,  \frac{1}{2}\for\Bt_2}, &
\mb_3 &=\mset{\frac{1}{8}\for\Bt_1, \frac{1}{4}\for\Bt_2, \frac{1}{2}\for\Bt_3}
\end{align*}
% 	\[
%\Bt_1 = [] \arrow \zero,\quad	\mb_1 =[\two \for\Bt_1]\quad\quad 
%\Bt_2=\mb_1\arrow  \zero, \quad\mb_2 = [\frac{1}{4} \for\Bt_1,  \frac{1}{2}\for\Bt_2], \quad\quad 
% \Bt_3=\mb_2\arrow   \zero, \quad \mb_3 = [\frac{1}{8}\for\Bt_1, \frac{1}{4}\for\Bt_2, \frac{1}{2}\for\Bt_3]
%	\]
The given types are structurally very similar to those from
Section~\ref{sec:examples_CbV}. We can thus mimick the constructions
given there, and get derivations $\Sigma_i$, each having weight $2$ and
typing $\mex$ with $\Bt_i$, but also derivations having weights
converging to $4$, this time typing $\mex\mex$ with $\zero$.
%The first thing to check is the way we can type the value
%$\mex=\lam x. xx \oplus I$. Actually, it can be given all
%the arrow types $\mb_i$ for every $i$, and in all cases
%the weight is $2$, i.e. there are proofs $\Sigma_i$ such that
%$\Sigma_i\dem\ovdash{2}\lam x. xx \oplus I: \Bt_i$. From
%the type derivations $\Sigma_i$'s, one can also attribute the intersection type
%$\Bt_i$ to $\mex$, this time with weight $\sum_{0\leq j<i}^i\frac{1}{2^j}=2-\frac{1}{2^{i-1}}$, obtaining
%the type derivation $\Theta_i$. Finally, $\Sigma_{i+1}$
%and $\Theta_i$ can be aggregated as follows, typing $\mex\mex$:
%\[
%\infer{\ovdash {4-\frac{1}{2^{i-1}} } \mex\mex:  \zero}
%      {\Sigma_{i+1}\dem\ovdash{2}\mex:  \mb_i\arrow \zero
%	&
%       \Theta_i\dem\ovdash{2-\frac{1}{2^{i-1}}} \mex: \mb_i
%      }
%\]
So for example, recalling that $\etime 6 {\mex\mex}= 3+\two$, here is
the corresponding type derivation:

{\footnotesize
\[
\infer{ \ovdash {3+\two} \mex\mex:  \zero }
	{\infer{\Sigma_3\dem\ovdash{2} \lam x.  xx\oplus I: [\two \for\Bt_2, \frac{1}{4}\for \Bt_1]\arrow 
			\zero}{
			\infer[\oplus]{x:[\two \for\Bt_2, \frac{1}{4}\for \Bt_1] \ovdash{1} xx\oplus I:  
				\zero }{
				\infer{x:[ \Bt_2, \two \for\Bt_1] \ovdash  0 xx:    \zero  }{
					x:[  [\two\for \Bt_1]\arrow    \zero  ] \ovdash 0 x:  [ [\two\for \Bt_1]\arrow    \zero   ]  
					& {x:[\two\for \Bt_1]\ovdash 0 x:[\two \for\Bt_1] }
				}
				&
				\infer{\ovdash  0 I: \zero }{}
			}
		} 
		&
		\infer[!]{\Sigma \dem \ovdash{1+\two} \mex:  [\frac{1}{2}\for \Bt_2, \frac{1}{4}\for\Bt_1]}
		{\Sigma_1 \dem  \ovdash {2} \mex:\Bt_1 & \Sigma_2 \ovdash{2} \mex:\Bt_2}    }
	\]}
        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Focusing on the Probability of Termination}\label{sec:focusAST}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we have shown that our type system induces
characterisations of both \AST and \PAST by \emph{the same} family of
derivations, namely the tight derivations.  Moreover, we proved that we
can restrict the search space to the class of null typings whenever
interested in the expected number of steps, only.  But there is more:
if we are interested in the probability of termination \emph{only}, an orthogonal
simplification is possible---we could drop from the typing all the
information on the scaling factors, as that is only used in
deriving the weight.
%\RED{This is coherent with the fact, proved in \cite{} that the
%complexity of establishing \AST and \PAST is \emph{orthogonal}.}
%\cf{This is coherent with the fact, proved in \cite{}, that establishing \AST and \PAST belongs to  \emph{orthogonal} 
%complexity classes.}



==> 05-CbN.tex <==
% !TEX root = main_PAST.tex

\renewcommand{\ss}{\ee}
\section{Call-by-Name}
In Section~\ref{} we have defined a typing system for the Call-by-Value calculus $\PLambda^\cbv$ which characterizes both  \AST and \PAST. In this section we show that 
similar results are possible  also for a Call-by-Name calculus.


As language we use here a rather standard probabilistic CbN $\lam$-calculus,  equipped with weak head reduction.
We first define the language,  called $\PLambda^\cbn$,  and its operational semantics, then the typing system.


\paragraph{Call-by-Name Calculus.}
\emph{Terms} and \emph{evaluation contexts} are defined  by the grammar

\begin{align*}
M&::=  x \mid \lambda x.M \mid MM \mid M \oplus M\qquad&\mbox{\textbf{Terms} $ \PLambda $}\\
\ss&::=  \hole{}  \mid \ss M   & \mbox{\textbf{Contexts}}
\end{align*}
%\begin{align}
%	\ss &::= \hole{~} \mid \ss M                  &   \mbox{\textbf{Contexts}}\\
%	M &::= M \mid  \lam x. M \mid M M \mid M \oplus M  & \mbox{\textbf{Terms}}
%\end{align}
where $x$ ranges over a countable set of \emph{variables}, $\hole{}$ denotes the \emph{hole} of the context.  Given a
context $\ss$, we denote by $\ss \hole M$ the term obtained from $\ss$ by
filling the hole with $M$, allowing the capture of free variables.
Value are defined as for $\PLambda^\cbv$



\paragraph{Operational Semantics.}As before, we first define one-step reduction $\red$ from terms to multidistributions. The rules are given in Figure~\ref{fig:reductions}. 
We  then lift  $\red$ to \emph{reduction of
	multidistributions} as in  Figure \ref{fig:lifting}.


	\begin{figure}\centering
	\fbox{
		\begin{minipage}{0.97\textwidth}\centering
			{\footnotesize 	$ 	{\ss \hole{(\lambda x.M)N }\redb \mdist{\ss\hole{ M \subs x } }}{	}
				\qquad
				{\ss\hole{M\oplus N} \red_{\oplus} \mdist{\frac{1}{2}\ss(M), \frac{1}{2}\ss(N)}}{} $		\qquad	
					$ \red\,:=\, \redb\cup \redo $
			}
	\end{minipage}}	\caption{Reduction Steps }\label{fig:reductions}
\end{figure}


\paragraph{Probabilistic Termination in $\PLambda^\cbn$}
Values  (like before, variable and abstractions) are are exactly the normal forms of the calculus.

The definition of  $ \nnorm {\m_k}$, $\eval k M$, $\ProbTerm M$,  $\etime k M$, an d$\ETime M$ are the same as in \ref{sec:}, and so the definition of \AST and \PAST.

\subsection{The CbN Typing System} Non-Idempotent Intersection types for Call-by-Name $\lam$-calculus have been introduced by \cite{Carvalho, **} and are well-studied.  We adapt them to our  probabilistic setting.

The types  reflect the behaviour of Call-by-Name, which is simpler than that   of CbV.
Like in the case of  $\PLambda^\cbv$, the type system is based on
{three}, rather than {two} layers, namely arrows,
intersection types, and multidistribution types.
Notice however that now  
a \emph{type distribution} is a (multi)-distribution over arrows. An \emph{intersection type} is a multiset of scaled types, \ie a multiset of pairs
$q\for \at$ where $\at$ is a type distribution, and $q\in ]0,1]\cap
\Qnum$ is a \emph{scale factor}.


%%%%%%%%%%%%%%%%%
Types are defined by means of the following grammar:
%
\begin{align*}
\At,\Bt & ::=  * \mid {\ma \arrow \at}  & {\mbox{ \textbf{Arrow Types}}}\\
\at,\bt & ::=  \mdist{p_{1}\At_{1},...,p_{n}\At_{n}}, n \geq 0 & \mbox{ \textbf{Types distribution} }\\
\mA,\mB & ::=  \mul{q_1\for \at_{1},...,q_n \for\at_{n}} n \geq 0 & \mbox{  \textbf{Intersection Types}}
\end{align*}
%\SLV{}{where $*$ is sugar for $[]\arrow \zero$.}
%
\paragraph{Typing rules.}
%%%%%%%%%%%%%%%%%%%%%%%%%
The type assignment system in Fig. \ref{fig:WWcbv} proves judgements
of the shape $\Gamma \oder w M: \type$, where $\Gamma$ is a type
context, $M$ a term, $w\in \Qnum $ is a  counter, and $\type$ is either $ \at$ or $\mA$.


\begin{figure}
	{\footnotesize 
		\fbox{\begin{minipage}{0.95\textwidth}
			{\footnotesize
				 	\[   \infer[var]{ x:\mset {1\for\at}  \ovdash 0 x:\at}{}  
				\quad\quad
				\infer[val]{ \ovdash 0  \lam x.M :\dist{*}}{}
				\quad \quad \infer[0]{  \oder{0 } M:\zero}{}
				\] 
				
						
				
				\[	\infer[\arrow I]{\Gamma \ovdash {w+1} \lam x. M: \dist{\ma \arrow \bt}}{\Gamma, x:\ma \ovdash {w} M:\bt} \quad \quad\quad
%				\infer[\arrow E]{\Pi\dem ~\Gamma  \uplus_k  \Delta_k \oder {w+ \sum_k w_k} MN: {\dsum_k~ p_k \bt_k}}
%				{\Pi_0\dem ~\Gamma \oder {w} M: \dist {p_k (\ma_k \arrow \bt_k) }_{\kK}&  
%					\big(\Pi_k\dem ~\Delta_k \oder {w_k} N: {p_k\for} \mA_k\big)_{k\in K}}	
				\infer[\arrow E]{\Gamma  \uplus_k  {p_k\for}\Delta_k \oder {w+ \sum_k p_k w_k} MN: {\dsum_k~ p_k \bt_k}}
				{\Gamma \oder {w} M: \dist {p_k (\ma_k \arrow \bt_k) }_{\kK}&  
					\big(\Pi_k\dem ~\Delta_k \oder {w_k} N:  \mA_k\big)_{k\in K}}	
				\]
				
							
				
				\[
				\infer[!]{\uplus_i (q_i\for\Gamma_i)\oder {\sum_i  q_i w_i} M:\mset{q_i\for\at_i\st \iI}}
				{(\Gamma_i\oder {w_i} M: \at_i)_{\iI}\quad &  \quad(q_i)_{\iI} \mbox{ scale factors}
				}
			\quad\quad\quad
				\infer[\oplus]{\two\for\Gamma \uplus \two\for\Delta \oder{1+\two w_1 +\two w_2} M\oplus N: \two \at \dsum \two \bt}
				{\Gamma \oder {w_1} M: \at & \Delta \oder{w_2} N: \bt} 
				\]
				}
				
				\begin{itemize}
					\item $ u\for [q_1\for\at_1, \dots, q_k\for\at_k] =[(u q_1)\for\at_1, \dots, (u q_k)\for\at_k] $
					\item 	If $\Gamma = x_1:\mA_1, \dots, x_j:\mA_j$, then $q\for \Gamma = x_1:q\for\mA_1, \dots, x_j:q\for \mA_j$
				\end{itemize}
				\caption{ CbN type assignment system  }\label{fig:WWcbn}
		\end{minipage}}	
	}
\end{figure}


%\begin{Def}[Tight Types and Derivations]
%	A type $\at$ is said to be \emph{tight} if it is a multidistribution
%	on the arrow $* \deff []\arrow \zero$. Accordingly, a derivation
%	$\Pi\dem ~ \oder w M: \at $ is said to be \emph{tight} if $\at$ is tight.
%\end{Def}

\begin{Def}[Tight types and  derivations] 	A \emph{type} $\at$ is said to be \emph{tight} if it is a multidistribution
		on the arrow type $*$. A derivation $\Pi\dem ~ \oder w M: \at $ is   tight if $\at$ is tight.
\end{Def}

\SLV{}{
Note that the following is easily  derived rule:
\[\infer[val]{ \oder 0  \lam x.M :\dist{*}}{}\]


\begin{property}[Closed values] Any closed value $\lam x.M$ can be  tightly typed  with probability $1$ by $ \oder 0  \lam x.M :\dist{*} $.

\end{property}
}

\paragraph{Properties.} 
\begin{itemize}
	
	\item Closed values. Any closed value $\lam x.M$ can be  tightly typed  with probability $1$, by $ \oder 0  \lam x.M :\dist{*} $.
	
%	\item ($\arrow I$) Vacuous abstractions: we  can  always abstract a variable $x$ which does not explicitly occur in the context $\Gamma$. Indeed, if  $x \not\in dom (\Gamma)$, then $\Gamma, x :[]$ is equal to $\Gamma$.
%	
	\item ( $!$-rule). Taking $K=\emptyset$, the following   \emph{holds for any term} $M$ \[\infer{\oder{0} M:[~]}{}\]
	
	\item  ($\arrow E$ rule). If  $K=\emptyset$,  we have 
	\[\infer{\Gamma \oder {w} MN:\zero}{\Gamma \oder{w} M:\zero }				
	\]
	
	
\end{itemize}
\subsection{Characterizing CbN Probabilistic Termination}
The typing system allows us to obtain exactly the same results we had for $\PLambda^\cbv$.  Finitary soundness  and finitary completeness both hold, exactly  as in Theorem~\ref{th:correct} and Theorem~\ref{th:complete}. The statement is the same, taking into account that now $M$ is a closed term of $\PLambda^\cbn$. As a consequence, we can 
\begin{itemize}
	\item characterize \AST and \PAST in a uniform way, via \emph{tight typing}, exactely as in Theorem~\ref{th:term_tight} and Corollary~\ref{cor:char_tight}, and 
	\item characterize \PAST simply via \emph{null typing}, 
this time exactly like in Theorem~\ref{thm:char_null}.
\end{itemize}
As we said in Section~\ref{}, one can also obtain a (simpler) 
 type system for \AST 
by dropping   from the typing all the
information on the scaling factors. \blue{A similar CbN typing  system is presented in \cite{RonchiDalLagoFaggian}.}


==> 99_Typing.tex <==
\newpage
\section{A cleaner typing}
\begin{figure}[!h]
	{\small 
		\fbox{\begin{minipage}{0.9\textwidth}
				\[
				\infer[ax]{ x: \mA  \ovdash 0 x:\mA}{}  
				\quad\quad
				\infer[0]{  \oder{0 } M:\zero}{}
				\]
				\[
				\infer[@]{\Gamma  \uplus  \Delta \oder {\RED{w+ w'+1}} VW: {\bt}}
				{\Gamma \oder {w} V: [\mA\arrow \bt]   & \Delta\oder {w'} W: \mA}	
				\qquad
				\infer[\oplus]{\two\for\Gamma \uplus \two\for\Delta \oder{\two w_1 +\two w_2 + 1} M\oplus N: \two \at \dsum \two \bt}
				{\Gamma \oder {w_1} M: \at & \Delta \oder{w_2} N: \bt} 
				\]
				\[
				\infer[\lam]{\Gamma \ovdash {w} \lam x. M: \mA \arrow \bt}
				{\Gamma, x:\mA \ovdash {w} M:\bt}  
				\quad\quad        
				\infer[\letr]{\Gamma  \uplus_k  p_k\for\Delta_k \oder {\RED{ \sum_k p_k w_k+ w+1}} \lett  N M: {\dsum_k~ p_k \bt_k}}
				{	(\Delta_k,  x:  \mA_k\oder {w_k} M: \bt_k)_{k\in K}	   &\Gamma \oder {w} N: \dist { p_k \mA_k }_{\kK}  	}	
				\]
				\[
				\infer[val]{\Gamma\oder {w} V:\dist{\mA} }{\Gamma\oder {w} V:\mA}
				\quad\quad
				\infer[!]{\uplus_i (q_i\for\Gamma_i)\oder {\sum_i  q_i w_i} V:\mset{q_i\for\At_i}_{\iI}}
				{(\Gamma_i\oder {w_i} V: \At_i)_{\iI}\quad &  \quad(q_i)_{\iI} \mbox{ scale factors}
				}
				\]              
	\end{minipage}}}
	\caption{Monadic Non-Idempotent Intersection Type Rules}
\end{figure}

\begin{figure}[!h]
	{\footnotesize 
		\fbox{\begin{minipage}{0.95\textwidth}
				{\footnotesize
					\[   \infer[var]{ x:\mset {1\for\at}  \ovdash 0 x:\at}{}  
					\quad\quad
					\quad \quad \infer[0]{  \oder{0 } M:\zero}{}
					\] 
					
					
					
					\[	\infer[\arrow I]{\Gamma \ovdash {w} \lam x. M: \dist{\ma \arrow \bt}}{\Gamma, x:\ma \ovdash {w} M:\bt} \quad \quad\quad
					%				\infer[\arrow E]{\Pi\dem ~\Gamma  \uplus_k  \Delta_k \oder {w+ \sum_k w_k} MN: {\dsum_k~ p_k \bt_k}}
					%				{\Pi_0\dem ~\Gamma \oder {w} M: \dist {p_k (\ma_k \arrow \bt_k) }_{\kK}&  
					%					\big(\Pi_k\dem ~\Delta_k \oder {w_k} N: {p_k\for} \mA_k\big)_{k\in K}}	
					\infer[\arrow E]{\Gamma  \uplus_k  {p_k\for}\Delta_k \oder {\RED{w+ \sum_k p_k w_k +1}} MN: {\dsum_k~ p_k \bt_k}}
					{\Gamma \oder {w} M: \dist {p_k (\ma_k \arrow \bt_k) }_{\kK}&  
						\big(\Pi_k\dem ~\Delta_k \oder {w_k} N:  \mA_k\big)_{k\in K}}	
					\]
					
					
					
					\[
					\infer[!]{\uplus_i (q_i\for\Gamma_i)\oder {\sum_i  q_i w_i} M:\mset{q_i\for\at_i\st \iI}}
					{(\Gamma_i\oder {w_i} M: \at_i)_{\iI}\quad &  \quad(q_i)_{\iI} \mbox{ scale factors}
					}
					\quad\quad\quad
					\infer[\oplus]{\two\for\Gamma \uplus \two\for\Delta \oder{\two w_1 +\two w_2+1} M\oplus N: \two \at \dsum \two \bt}
					{\Gamma \oder {w_1} M: \at & \Delta \oder{w_2} N: \bt} 
					\]
				}
				
%				\begin{itemize}
%					\item $ u\for [q_1\for\at_1, \dots, q_k\for\at_k] =[(u q_1)\for\at_1, \dots, (u q_k)\for\at_k] $
%					\item 	If $\Gamma = x_1:\mA_1, \dots, x_j:\mA_j$, then $q\for \Gamma = x_1:q\for\mA_1, \dots, x_j:q\for \mA_j$
%				\end{itemize}
				\caption{ CbN type assignment system  }
		\end{minipage}}	
	}
\end{figure}

==> DATI.tex <==
7CCE42D59922374D21D15E1572


4225C0070610053

19690331



==> macro_spazio.tex <==

%\parskip=0pt plus 1pt
%\setlength\parskip{0pt plus 1pt}
%\setlength\parskip{1em plus 0.1em minus 0.2em}

\usepackage{atbeginend}

%%%%%%%%%%%%%%%%%%%%


%\BeforeBegin{example}{\vspace{-6pt}}
%\BeforeEnd{example}{\vspace{-4pt}}
%\AfterEnd{example}{\vspace{-2pt}}

%\AfterBegin{example}{\vspace{-4pt}}
%\BeforeEnd{example}{\vspace{-4pt}}

%\AfterBegin{center}{\vspace{-8pt}}
%\BeforeEnd{center}{\vspace{-4pt}}



\AfterBegin{figure}{\vspace{-2pt}}
\BeforeEnd{figure}{\vspace{-8pt}}




%%%%%%%%%%%%%%%%%%%
%\theoremstyle{plain}
%\newtheorem{Def}[theorem]{Definition}
%\newtheorem{thm}[theorem]{Theorem}
%\newtheorem{prop}[theorem]{Proposition}
%\newtheorem{lem}[theorem]{Lemma}
%\newtheorem{cor}[theorem]{Corollary}
%\newtheorem{notation}[theorem]{Notation}
%\newtheorem{fact}[theorem]{Fact}
%\newtheorem{rem}[theorem]{Remark}
%
%\newtheorem*{theorem*}{Thm}
%\newtheorem*{proposition*}{Prop}
%\newtheorem*{lemma*}{Lemma}
%\newtheorem*{ex*}{Example}



%%
%\BeforeBegin{thm}{\vspace{-2pt}}
%\BeforeEnd{thm}{\vspace{-2pt}}
%\BeforeBegin{theorem}{\vspace{-2pt}}
%\BeforeEnd{theorem}{\vspace{-2pt}}
%\BeforeBegin{Def}{\vspace{-2pt}}
%\BeforeEnd{Def}{\vspace{-2pt}}
%\BeforeBegin{prop}{\vspace{-2pt}}
%\BeforeEnd{prop}{\vspace{-2pt}}
%\BeforeBegin{lem}{\vspace{-2pt}}
%\BeforeEnd{lem}{\vspace{-2pt}}
%\BeforeBegin{lemma}{\vspace{-2pt}}
%\BeforeEnd{lemma}{\vspace{-2pt}}
%\BeforeEnd{cor}{\vspace{-2pt}}
%\BeforeBegin{fact}{\vspace{-2pt}}
%\BeforeEnd{fact}{\vspace{-2pt}}
%\BeforeBegin{notation}{\vspace{-2pt}}
%\BeforeEnd{notation}{\vspace{-2pt}}
%\BeforeBegin{rem}{\vspace{-2pt}}
%\BeforeEnd{rem}{\vspace{-2pt}}
%
%
%\BeforeBegin{theorem*}{\vspace{-2pt}}
%\BeforeEnd{theorem*}{\vspace{-2pt}}
%\BeforeBegin{lemma*}{\vspace{-2pt}}
%\BeforeEnd{lemma*}{\vspace{-2pt}}
%\BeforeBegin{cor}{\vspace{-2pt}}
%\BeforeEnd{cor}{\vspace{-2pt}}
%
%
%\BeforeBegin{definition}{\vspace{-2pt}}
%\BeforeEnd{definition}{\vspace{-2pt}}
%


